Fairness for Workers Who Pull the Arms: An Index Based Policy for Allocation of Restless Bandit Tasks

Motivated by applications such as machine repair, project monitoring, and anti-poaching patrol scheduling, we study intervention planning of stochastic processes under resource constraints. This planning problem has previously been modeled as restless multi-armed bandits (RMAB), where each arm is an intervention-dependent Markov Decision Process. However, the existing literature assumes all intervention resources belong to a single uniform pool, limiting their applicability to real-world settings where interventions are carried out by a set of workers, each with their own costs, budgets, and intervention effects. In this work, we consider a novel RMAB setting, called multi-worker restless bandits (MWRMAB) with heterogeneous workers. The goal is to plan an intervention schedule that maximizes the expected reward while satisfying budget constraints on each worker as well as fairness in terms of the load assigned to each worker. Our contributions are two-fold: (1) we provide a multi-worker extension of the Whittle index to tackle heterogeneous costs and per-worker budget and (2) we develop an index-based scheduling policy to achieve fairness. Further, we evaluate our method on various cost structures and show that our method significantly outperforms other baselines in terms of fairness without sacrificing much in reward accumulated.

==> Fair Restless Bandits/adjusted_index_algo.tex <==







\subsection{Adjusting for interaction effects}
\label{sec:adjusted_index}


%Thus far, on a given arm $i$, our index computation for each worker $j$ relied on decomposing the MDP$_i$ down to multiple two-action MDPs, each with actions $0$ and $j$ for each worker $j\in[M]$. %Let us denote each two-action MDP for a given $j$ as $\langle S_i, A^j_i, C^j_i, P^j_i, R_i\rangle$, where $A^j_i = \{0, j\}$, $C^j_i = [0, c_{ij}]$ and $P^j_i$ is $P_i$ restricted to the $j^{th}$ two-action domain, i.e., $P^j_i:S_i \times A^j_i \times S_i \rightarrow{} \Delta^{|S^i|}$. This allows us to use existing techniques for computing Whittle indices, such as via binary search. 
%However, unlike traditional two-action RMABs, 
The indices obtained using Alg.~\ref{alg:WI} are not indicative of the true long-term value of taking that action in the MWRMAB problem. This is because, for a given arm, the value of an intervention by worker $j$ in general depends on interventions by other workers $j^\prime$ at different timesteps. %This inter-action dependence cannot be captured with only Step 1. 

Consider a MWRMAB corresponding to an anti-poaching patrol planning problem with 2 workers, where each worker is a type of ``specialist'' with different equipment (detailed in Fig.~\ref{fig:decoupled_counterexample}). 
    \begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/decoupled_counterexample_fig_new.pdf}
    \caption{Specialist domain: where specific actions are required in each state to advance to the reward-giving state. Decoupled indices lead to sub-optimal policies, whereas adjusted indices perform well.}
    \label{fig:decoupled_counterexample}
    \end{figure}

The first ranger (worker), $a_1$, has special equipment for clearing overgrown brush, and the second ranger, $a_2$, has specialized equipment for detecting snares, e.g., a metal detector. Assume $3$ states for each patrol area $i$ as ``overgrown and snared'' ($s=0$), ``clear and snared'' ($s=1$), and ``clear and not snared'' ($s=2$). Assume that reward is received only for arms in state $s=2$, and that snares cannot be cleared from areas with overgrown brush, i.e., $P^{02}_{ij}=0\ \forall j \in [M]$. If we assume that each worker is a ``true'' specialist--- so, ranger 1's equipment is ineffective at detecting snares, i.e., $P^{12}_{i1}=0$, and ranger 2's equipment is ineffective at clearing overgrown brush, i.e., $P^{01}_{i2}=0$ --- then the optimal policy is for ranger 1 to act on the arm in state ``overgrown and snared'' and ranger 2 to act on the arm in state ``clear and snared''. However, the fully decoupled index computation for each ranger $j$ would reason about restricted MDPs that only have passive action and ranger type $j$ available. So when computing, e.g., the index for ranger 1 in $s=0$, the restricted MDP would have $0$ probability of reaching state ``clear and not snared'', since it does not include ranger 2 in its restricted MDP. This would correspond to an MDP that always gives 0 reward, and thus would artificially force the index for ranger 1 to be $0$, despite ranger 1 being the optimal action for $s=0$. 

% The above procedure computes indices in a manner that fully decouples arms and workers. That is, the index for any given worker, arm pair does not reason about possible intervention effects that could be provided by other workers. The primary benefit of such a computation is its speed. We would expect those indices to perform well for such cases where intervention effects of some worker dominate those for other workers on a given arm, meaning the optimal policy for that arm would only utilize actions from that best worker anyway. It is straightforward to show that this is the case for 2-state problems. However, for problems with more than 2 states, it can be problematic to develop index estimates for each action that do not consider inter-action affects -- that is, policies which utilize different actions in different states.


% Consider a 3-state 2-worker MWRMAB corresponding to a machine-repair problem, where each worker is a type of specialist (visualized in Fig.~\ref{fig:decoupled_counterexample}). Specifically, let the first worker be a hardware specialist, and the second worker be a software specialist. Let the states be ``broken hard drive'' (state 0), ``needs new operating system'' (state 1), and ``functioning normally'' (state 2). Assume that reward is received only for arms in state 2 and that all machines with broken hard drives need new operating systems. If we assume that each worker is a ``true'' specialist ---i.e., worker 1 is ineffective at fixing software problems, and worker 2 is ineffective at fixing hardware problems --- then the optimal policy is for worker 1 to act on the arm in state ``broken hard drive'' and worker 2 to act on the arm in state ``needs new operating system''. However, the fully decoupled index computation for each worker $j$ would reason about restricted MDPs that only have passive action and worker type $j$ available. So when computing, e.g., the index for worker 1 in state 0, the restricted MDP would have no transition probabilities that could lead to state ``functioning normally'', since it does not include worker type 2 in its restricted MDP. This would correspond to an MDP that always gives 0 reward, and thus would artificially force the index to be 0, despite worker 1 being the optimal action.

To address this, we define a new index notion that accounts for such inter-action effects. The key idea is that, when computing the index for a given worker, we will consider actions of \textit{all other workers in future time steps.} So in our poaching example, the new index value for ranger 1 in $s=0$ will \textit{increase} compared to its decoupled index value, because the new index will take into account the value of ranger 2's actions when the system progresses to $s=1$ in the future. Note that the methods we build generalize to any number of workers $M$. However, the manner in which we incorporate the actions of other workers must be done carefully, We propose an approach and provide theoretical results explaining why. Finally, we give the full algorithm for computing the new indices.

\textbf{New index notion}: For a given arm, to account for the inter-worker action effects, we define the new index for an action $j$ as the minimum charge that makes an intervention by $j$ on that arm as valuable as \textit{any} other worker $j^\prime$ in the combined MDP, with $M+1$ actions. That is, we seek the minimum charge for action $j$ that makes us indifferent between taking action $j$ and \textit{not} taking action $j$, a multi-worker extension Whittle's index notion. %We propose to account for these inter-action effects by, for a given arm $i$, expanding the MDP which is used to compute the index for action $j$. Specifically, we will consider the MDP corresponding to the per-arm subproblem in Eq.~\ref{eq:RMAB_lagrange_sub}, which is identical to a given arm's unrelaxed MDP, except that a charge $\lambda_{ij^\prime}c_{ij^\prime}$ is applied for taking action $j^\prime$. That is, $P_i$ retains its unrestricted domain, but we define 
% In this section, we focus on only one arm, so we drop the subscript $i$.
To capture this, we define an augmented reward function $R^{\dagger}_{\bm{\lambda}}(s,j) = R(s) - \lambda_{j} c_{{j}}$. Let $\bm{\lambda}$ be the vector of $\{\lambda_{j}\}_{j\in[M]}$ charges. We define this \textbf{expanded MDP} as $\mathcal{M}^{\dagger}_{\bm{\lambda}}$ %:= \langle S, A, C, P, R^{\dagger}_{i, \bm{\lambda}_i}\rangle$, with 
and the corresponding value function as $V^{\dagger}_{\bm{\lambda}}$. We now find adjusted index $\lambda^{adj,*}_{j,\bm{\lambda}_{-j}}$ using the following expression: % which captures the value of taking action $j$ in the expanded MDP where $\bm{\lambda}_{i,-j}$ is a vector of fixed charges $\lambda_{ij^\prime} c_{i{j^\prime}} \forall j^\prime \ne j$, but the charge $\lambda_{ij}$ for action $j$ is varied. Formally, for a given arm $i$, charges $\bm{\lambda}_i$, state $s$, and worker $j$, we define the adjusted index value as:
\begin{align}
    \label{def:adjusted_index}
    %\lambda^{adj,*}_{ij,\bm{\lambda}_{i,-j}}&(s) = \nonumber \\ 
    \min_{j'\in[M]\setminus\{j\}}\arg\min_{\lambda_{j}}\{\lambda_j\!\!:\!\!\ V^{\dagger}_{\bm{\lambda}_{-j}}(s,\lambda_j,j)=V^{\dagger}_{\bm{\lambda}_{-j}}(s,\lambda_j,j^\prime)\}
\end{align}
%We now drop the subscript $i$ where it is unambiguous. 
where $\bm{\lambda}_{-j}$ is a vector of fixed charges for all  $j^\prime \ne j$, and the outer $\min$ over $j^\prime$ simply captures the specific action $j^\prime$ that the optimal planner is indifferent to taking over action $j$ at the new index value. %, but the charge $\lambda_{j}$ for action $j$ is varied.
Note, this is the natural extension of the decoupled two-action index definition, Eq.~(\ref{def:decoupled_index}), which defines the index as the charge on $j$ that makes the planner indifferent between acting and, the only other option, being passive.
% , Eq.~(\ref{def:adjusted_index}) extends this definition to account for multiple actions, defining the index as the charge that makes the planner indifferent between taking action $j$ and taking some other action $j^\prime$. 
% The underlying intuitions for both types of indices are similar -- each index value captures the long-term  value of playing action $j$, considering the optimal policy with given other actions and charges, starting from the current state $s$. 
Our new \emph{adjusted index algorithm} is given in Alg.~\ref{alg:AIC}.

\begin{algorithm}[!h]
\small{
\caption{Adjusted Index Computation}\label{alg:AIC}
{\textbf{Input}: An arm: MDP $\mathcal{M}^{\dagger}$, costs $c_{j}$, state $s$, and indices $\lambda^{*}_{j}(s).\qquad\qquad$} 
% \textbf{Output}: Adjusted indices $\lambda^{adj,*}_{j}(s)$ for all workers $j\in[M]$ and state $s$ for the given arm. 
\begin{algorithmic}[1] %[1] enables line numbers
\FOR{$j=1$ to $M$}
\STATE $\bm{\lambda}_{j} = \lambda^{*}_{j}(s)$ \COMMENT{init $\bm{\lambda}$}
\ENDFOR
\FOR{$j=1$ to $M$}
% \STATE $\bm{c}^{adj} = [c_{i0}, c_{i1},\ldots,c_{iM}]$
% \FOR{$j^\prime = 1$ to $M$ s.t.~$j^\prime \ne j$}
% \STATE $\lambda_{j^\prime} = \lambda^{*}_{ij^\prime}(s_i)$
% \STATE $\bm{c}^{adj}[j^\prime] \leftarrow \bm{c}^{adj}[j^\prime]*\lambda_{j^\prime}$ \\
% \ENDFOR
\STATE Compute $\lambda^{adj,*}_{j,\bm{\lambda_{-j}}}(s)$ \COMMENT{via binary search on Eq.~\ref{def:adjusted_index}}
\ENDFOR
\STATE \textbf{return} $\lambda^{adj,*}_{j,\bm{\lambda_{-j}}}(s)$ for all workers $j\in[M]$
\end{algorithmic}
}
\end{algorithm}

We use a binary search procedure to compute the adjusted indices since $V^{\dagger}_{\bm{\lambda}_{-j}}(s,\lambda_j,j)$ is convex in $\lambda_j$. The most important consideration of the adjusted index computation is how to set the charges $\lambda_{j^\prime}$ of the other action types $j^\prime$ when computing the index for action $j$. We show that a reasonable choice for $\lambda_{j^\prime}$ is the Whittle Indices $\lambda^{*}_{j^\prime}(s)$ which were pre-computed using Alg.~\ref{alg:WI}. The intuition is that $\lambda^{*}_{j^\prime}(s)$ provides a \textit{lower bound} on how valuable the given action $j^\prime$ is, since it was computed against no-action in the restricted two-action MDP. In Observation~\ref{obs} and Theorem~\ref{thm:lam_0}, we describe the problem's structure to motivate these choices.

The following observation explicitly connects decoupled indices and adjusted indices.
\begin{observation}\label{obs}
For each worker $j$, when  $\bm{\lambda}_{-j}\rightarrow{}\infty$, i.e., $\lambda_{j^\prime} \rightarrow{}\infty \hspace{2mm} \forall j^\prime \ne j$, then the following holds: 
$\lambda^{adj,*}_{j,\bm{\lambda}_{-j}} \rightarrow{} \lambda^{*}_{j}$.
\end{observation}

This can be seen by considering the rewards $R^{\dagger}_{\bm{\lambda}}(s,j^\prime) = R(s) - \lambda_{j^\prime} c_{{j^\prime}}$ for taking action $j^\prime$ in any state $s$. As the charge $\lambda_{j^\prime}\rightarrow{}\infty$, $R^{\dagger}_{\bm{\lambda}}(s,j^\prime)\rightarrow{}-\infty$, making it undesirable to take action $j^\prime$ in the optimal policy. Thus, the optimal policy would only consider actions $\{0,j\}$, which reduces to the restricted MDP of the decoupled index computation.

Next we analyze a potential naive choice for $\bm{\lambda}_{-j}$ when computing the indices for each $j$, namely, $\bm{\lambda}_{-j} = 0$. Though it may seem a natural heuristic, this corresponds to planning \textit{without considering the costs of other actions}, which we show below can lead to arbitrarily low values of the indices, which subsequently can lead to poorly performing policies.
\begin{theorem}
\label{thm:lam_0}
As $\lambda_{j^\prime} \rightarrow{} 0 \hspace{2mm} \forall j^\prime \ne j$, $\lambda^{adj,*}_j$ will monotonically decrease, if (1) $V_{\lambda_{j^\prime}}^{\dagger}(s,\lambda_j,j^\prime) \ge V_{\lambda_{j^\prime}}^{\dagger}(s,\lambda_j,0)$ for 0 $\le \lambda_{j^\prime} \le \epsilon$ and (2) if the average cost of worker $j^\prime$ under the optimal policy starting with action $j^\prime$ is greater than the average cost of worker $j^\prime$ under the optimal policy starting with action $j$.
\end{theorem}
Thm.~\ref{thm:lam_0} %(proof in the arXiv version)
(proof in Appendix~\ref{sec:proof}) 
confirms that, although setting $\lambda_{j^\prime}=0$ for all $j^\prime$ may seem like a natural option, in many cases it will artificially reduce the index value for action $j$. This is because $\lambda_{j^\prime}=0$ corresponds to planning as if action $j^\prime$ comes with \textit{no charge}. Naturally then, as we try to determine the \textit{non-zero} charge $\lambda_j$ we are willing to pay for action $j$, i.e., the index of action $j$, \textit{we will be less willing to pay higher charges, since there are free actions $j^\prime$}. Note that conditions (1) and (2) of the above proof are not restrictive. The first is a common epsilon-neighborhood condition, which requires that value functions do not change in arbitrarily non-smooth ways with $\lambda$ values near 0. The second requires that a policy's accumulated costs of action $j^\prime$ are greater when starting with action $j^\prime$, than starting from any other action--- this is same as assuming that the MDPs do not have arbitrarily long mixing times. That is to say that Thm.~\ref{thm:lam_0} applies to a wide range of problems that we care about.

The key question then is: what are reasonable values of charges for other actions $\bm{\lambda}_{-j}$, when computing the index for action $j$? We propose that a good choice is to set each $\lambda_{j^\prime} \in \bm{\lambda}_{-j}$ to its corresponding decoupled index value for the current state, i.e., $\lambda^{*}_{j^\prime}(s)$. % which were pre-computed using the decoupled method. The idea is that $\lambda^{*}_{j^\prime}(s)$ provides a reasonable \textit{lower bound} on how valuable the given action $j^\prime$ is, since it was computed in the restricted two-action MDP. Correspondingly, that makes it a reasonable amount to charge for taking that action in the \textit{expanded} MDP, when computing the adjusted indices for other actions. 
The reason relies on the following key idea: we know that at charge $\lambda^{*}_{j^\prime}(s)$, the optimal policy is indifferent between choosing that action $j^\prime$ and the passive action, at least when $j^\prime$ is the only action available. Now, assume we are computing the new adjusted index for action $j$, when combined in planning with the aforementioned action $j^\prime$ at charge $\lambda^{*}_{j^\prime}(s)$. Since the charge for $j^\prime$ is already set at a level that makes the planner indifferent between $j^\prime$ and being passive, if adding $j^\prime$ to the planning space with $j$ does not provide any additional benefit over the passive action, \textit{then the new adjusted index for $j$ will be the same as the decoupled index for $j$, which only planned with $j$ and the passive action}. This avoids the undesirable effect of getting artificially reduced indices due to under-charging for other actions $j^\prime$, i.e., Thm.~\ref{thm:lam_0}. The ideas follow similarly for whether the adjusted index for $j$ should increase or decrease relative to its decoupled index value. I.e., if \textit{higher} reward can be achieved when planning with $j$ and $j^\prime$ together compared to planning with either action alone, as in the specialist anti-poaching example
% , then at a reasonable charge for action $j^\prime$ (i.e., $\lambda^\star_{j^\prime}(s)$) which indicates that we cannot rely \textit{solely} on $j^\prime$, 
then we will become \textit{more willing to pay a charge $\lambda_j$} now to help reach states where the action $j^\prime$ will let us achieve that higher reward. On the other hand, if $j^\prime$ dominates $j$ in terms of intervention effect, then even at a reasonable charge for $j^\prime$, we will be less willing to pay for action $j$ when both options are available, and so the adjusted index will decrease. 
% Given these ideas, we hypothesize that the index values following from these adjustments should lead to policies that more closely match the optimal when combined with a greedy-based index selection approach. 
We give our new \emph{adjusted index algorithm} in Alg.~\ref{alg:AIC}, and provide experimental results demonstrating its effectiveness.
% policy is indifferent to that action and the passive action combined in planning with a given action of interest $j$, the index for action $j$ should increase---relative to its decoupled value---if the new optimal policy utilizes \textit{both actions} $j$ and $j^\prime$ and leads to greater reward --- that is, so long as we do not \textit{undercharge} for action $j^\prime$ (Thm.~\ref{thm:lam_0}). Specifically, by setting the charge for $j^\prime$ to its decoupled index value, we are charging at least as much as would make us indifferent to acting if the new action $j$ \textit{were not available}. And thus, if there is no positive inter-action effect when planning with $j$ and $j^\prime$ together, we will again be indifferent when choosing between $j^\prime$ and being passive. However, the decoupled index for $j$ already planned against the passive action --- so the index for $j$ will stay the same. Alternatively, if there is a positive inter-action effect to planning with $j$ and $j^\prime$ together, then there will be states in which we prefer $j^\prime$ over being passive, even at the charge $\lambda^{*}_{j^\prime}$ --- that additional benefit will manifest in our additional willingness to pay for $j$ in the current state, i.e., the adjusted index for $j$ will become higher than the decoupled index for $j$. By a similar logic, actions $j$ that are truly worse to take at the current state than some other actions $j^\prime$, even at their charge levels $\lambda^{*}_{j^\prime}$, should decrease. Thus, we hypothesize that the index values following from these adjustments should lead to policies that more closely match the optimal when combined with a greedy selection approach. We give our new \emph{adjusted index algorithm} in Alg.~\ref{alg:AIC}, and provide experimental results demonstrating its effectiveness.


\iffalse
\begin{proposition}
\label{prop:set_lam}
Cases exist where using our proposed algo provides the correct index ordering, compared to the decoupled algo.
\end{proposition}
\begin{proof}
TODO -- use the specialist example.
\end{proof}
\fi



% The key difference behind this algorithm is that, for a given arm, it reasons about \textit{all} workers in its future policy when computing the index for a given worker. The definition of the index is similar to that for the 2-action case -- the $\lambda$ charge at which the policy is indifferent between taking that action or taking any other action. Since it reasons about all workers at once, it is more computationally expensive, though provides more accurate indices.

% However, as indicated by the LP in Eq.~\ref{eq:RMAB_lagrange}, a key factor in developing informative indices for each action $j$ will be in the setting of the $\lambda_{j^\prime}$ terms for all other workers $j^\prime \ne j$. Note that this complication was avoided when computing decoupled 2-action indices. However, if we say, take a naive setting of $\lambda_{j^\prime}=0 \forall j^\prime$ then the optimal policy during the computation of the index for $j$ will assume that it will have unbudgeted access to all other actions in the future. This is the key tension that makes planning in RMAB so challenging, and clearly will lead to suboptimal indices. Instead, we must develop reasonable estimates for $\lambda_{j^\prime}$ that are informative of how restricted that particular action will be, based on its desirability to the rest of the population of arms. 

% To develop these estimates, we propose to leverage the decoupled indices we have already computed for each action. Since we know the decoupled indices are not precise, we use them to develop a heuristic estimate of $\lambda_{j^\prime}$ by setting $\lambda_{j^\prime}$ to be the value of the final index of worker $j^\prime$ played by an imagined greedy policy which fully exhausted its budget for that worker $j^\prime$ across all arms. In this way, $\lambda_{j^\prime}$ serves as a reasonable estimate for how restricted the resource $j^\prime$ will be, allowing our index computation for $j$ to make principled tradeoffs in its optimal policy about how much it can rely on access to that action $j^\prime$ in the future. We demonstrate the effectiveness of this algorithm empirically on the domains in Fig.~\ref{fig:decoupled_counterexample}.

==> Fair Restless Bandits/intro.tex <==

Restless multi-armed bandits (RMABs)~\cite{whittle1988restless} have been used for sequential planning, where a planner allocates a limited set of $M$ \textit{intervention resources} across $N$ \textit{independent heterogeneous arms} (Markov Decision processes) at each time step in order to maximize the long-term expected reward. The term \textit{restless} denotes that the arms undergo state-transitions even when they are not acted upon (with a different probability than when they are acted upon). RMABs have been receiving increasing attention across a wide range of applications such as maintenance \citep{abbou2019group}, recommendation systems~\cite{meshram2015restless},  anti-poaching patrolling~\citep{qian2016restless}, adherence monitoring~\citep{Akbarzadeh2019,mate2020collapsing}, and intervention planning~\cite{mate2021field,biswas2021learning,killian2023robust}.  %However, despite the wide applicability of RMABs, surprisingly, RMAB literature has so far ignored one key reality that \textbf{the interventions being planned are often carried out by a \textit{human workforce}}. 
Although, \textit{rangers} in anti-poaching, \textit{healthcare workers} in health intervention planning, and \textit{supervisors} in machine maintenance are all commonly cited examples of human workforce used as intervention resources, the literature has so far ignored one key reality that the human workforce is heterogeneous---each worker has their own workload constraints and needs to commit a dedicated time duration for intervening on an arm. Thus, it is critical to restrict intervention workload for each worker and balance the workload across them, while also ensuring high effectiveness (reward) of the planning policy. 



%To further push these models toward real-world deployment, \cite{nishtala2021selective} has focused on scaling issues %online learning \cite{biswas2021learning,avrachenkov2020whittle},
%and \cite{herlihy2021planning} considered quota-based fairness across arms. 

%The idea of a human workforce has several important consequences that require more expressiveness from the planning model, including the heterogeneity of intervention effects among worker-arm pairs, worker-specific workload constraints, and the idea of balanced work allocation. \textit{These ideas are critical to encode in the system both to protect workers as well as to improve efficiency in planning}.  % and thus, a critical gap remains in matching RMABs to real-world intervention planning settings. %That is, most RMAB assume all intervention resources are identical. However, i
% However, more generally, interventions are commonly carried out by a human workforce, where each worker has a budget and (possibly varying) costs for acting upon arms (restless bandit tasks). 
RMAB literature does not consider this heterogeneity and mostly focuses on selecting best arms assuming that all intervention resources (workers) are interchangeable, i.e., as from a single pool (homogeneous). However, planning with human workforce requires more expressiveness in the model, including heterogeneity in costs and intervention effects,  worker-specific load constraints, and balanced work allocation. 
One concrete example is \textit{anti-poaching intervention planning}~\cite{qian2016restless} with $N$ areas in a national park where timely interventions (patrols) are required to detect as many snares as possible across all the areas. These interventions are carried out by a small set of $M$ ranger. The problem of selecting a subset of areas at each time step (say, daily) has been modeled as an RMAB problem.  However, each ranger may  incur heterogeneous cost (e.g., distance travelled, when assigned to intervene on a particular area) and the total cost incurred by any ranger (e.g., \textit{total} distance traveled) must not exceed a given budget. Additionally, it is important to ensure that tasks are allocated fairly across rangers so that, for e.g., some rangers are not required to walk far greater distances than others. Adding this level of expressiveness to existing RMAB models is non-trivial.

%Heterogeneous workers have not been considered even in real-world deployments~\cite{mate2021field,bhattacharya2018restless} of RMAB solutions with application to health intervention planning, where it is crucial to be fair across the healthcare workers. 

To address this, we introduce the \textit{multi-worker restless multi-armed bandits} (MWRMAB) problem. Since MWRMABs are more general than the  classical RMABs, they are at least PSPACE hard to solve optimally~\citep{papadimitriou1994complexity}. RMABs with $k$-state arms require solving a combined MDP with $k^N$ states and $|M+1|^N$ actions constrained by a budget, and thus suffers from the curse of dimensionality. A typical approach is to compute Whittle indices~\citep{whittle1988restless} for each arm and choose $M$ arms with highest index values---an asymptotically optimal solution under the technical condition \textit{indexability}~\citep{weber1990index}. However, this approach is limited to instances a single type of intervention resource incurring one unit cost upon intervention. A few papers on RMABs~\citep{glazebrook2011general,meshram2020simulation} study multiple interventions and non-unitary costs but assumes one global budget (instead of per-worker budget).  Existing solutions aim at maximizing reward by selecting arms with highest index values that may not guarantee fairness towards the workers who are in charge of providing interventions. 

\paragraph{Our contributions} To the best of our knowledge, we are the first to introduce and formalize the multi-worker restless multi-armed bandit (MWRMAB) problem and a related worker-centric fairness constraint. We develop a novel framework for solving the MWRMAB problem. Further, we empirically evaluate our algorithm to show that it is fair and scalable across a range of experimental settings.

%\begin{itemize}[topsep=0em,leftmargin=*,itemsep=0.05mm]
%    \item We introduce and formalize the multi-worker restless multi-armed bandit (MWRMAB) problem and a related worker-centric fairness constraint.
%    \item We develop a novel framework for solving the MWRMAB problem. %We establish conditions under which they perform well and derive a novel method for efficiently computing the indices in decomposable cases. 
%    We provide an index-based heuristic and an allocation strategy that achieves worker-centric fairness.
%    \item We empirically analyze our algorithms and demonstrate their effectiveness and superior real-world scalability across a range of experimental settings.
%\end{itemize}



